Rationals vs Byzantines in Consensus-based Blockchains

In this paper we analyze from the game theory point of view Byzantine Fault Tolerant blockchains when processes exhibit rational or Byzantine behavior. Our work is the first to model the Byzantine-consensus based blockchains as a committee coordination game. Our first contribution is to offer a game-theoretical methodology to analyse equilibrium interactions between Byzantine and rational committee members in Byzantine Fault Tolerant blockchains. Byzantine processes seek to inflict maximum damage to the system, while rational processes best-respond to maximise their expected net gains. Our second contribution is to derive conditions under which consensus properties are satisfied or not in equilibrium. When the majority threshold is lower than the proportion of Byzantine processes, invalid blocks are accepted in equilibrium. When the majority threshold is large, equilibrium can involve coordination failures , in which no block is ever accepted. However, when the cost of accepting invalid blocks is large, there exists an equilibrium in which blocks are accepted iff they are valid.

==> decisionTree.tex <==
% !TeX root = main.tex

\begin{figure}
	\center
%	\resizebox{\linewidth}{!}{
	\begin{tikzpicture}[grow=right, sloped]
	\node[bag]{}
%	child{
%	\node[bag]{Proposer is rational}
%	child{
%	node[bag] {Proposal valid}%{Bag 1 $4W, 3B$}
	    child {
	        node[bag] {Does not check the validity}        
	            child {
	                node[bag] {\textit{No Validity Information}}
	                child{
	                	node[end, label=right: Not Send] {}
	            		edge from parent 
	                } child{
	                	node[end, label=right: Send] {}
	          		edge from parent 
	                }
	                edge from parent
	            }
	            edge from parent 
	%            node[above] {$W$}
	%            node[below]  {$\frac{4}{7}$}
	    }
	    child {
	        node[bag] {Checks the validity}        
	            child {
	                node[bag] {\textit{Not Valid}}
	                child{
	                	node[end, label=right: Not Send] {}
	            		edge from parent 
	                } child{
	                	node[end, label=right: Send] {}
	          		edge from parent 
	                }
	                edge from parent
	            }        
	            child {
	                node[bag] {\textit{Valid}}
	                child{
	                	node[end, label=right: Not Send] {}
	            		edge from parent 
	                } child{
	                	node[end, label=right: Send ] {}
	          		edge from parent 
	                }
	                edge from parent
	            }
	        edge from parent
	    }
%	    edge from parent
%	    }
%	    edge from parent
%	    }
%	    
%	    child{
%	    node[bag]{Proposer is symmetric Byzantine}
%	    child{
%	    node[bag] {Proposal inalid}%{Bag 1 $4W, 3B$}
%	    child {
%	        node[bag] {Does not check the validity}        
%	            child {
%	                node[bag] {No Validity Information}
%	                child{
%	                	node[end, label=right: Not Send] {}
%	            		edge from parent 
%	                } child{
%	                	node[end, label=right: Send] {}
%	          		edge from parent 
%	                }
%	                edge from parent
%	            }
%	            edge from parent 
%	%            node[above] {$W$}
%	%            node[below]  {$\frac{4}{7}$}
%	    }
%	    child {
%	        node[bag] {Checks the validity}        
%	            child {
%	                node[bag] {Not Valid}
%	                child{
%	                	node[end, label=right: Not Send] {}
%	            		edge from parent 
%	                } child{
%	                	node[end, label=right: Send] {}
%	          		edge from parent 
%	                }
%	                edge from parent
%	            }        
%	            child {
%	                node[bag] {Valid}
%	                child{
%	                	node[end, label=right: Not Send] {}
%	            		edge from parent 
%	                } child{
%	                	node[end, label=right: Send] {}
%	          		edge from parent 
%	                }
%	                edge from parent
%	            }
%	        edge from parent
%	    }
%	    edge from parent
%	    }
%	    edge from parent
%	    } 
	    ;
	\end{tikzpicture}
%	}
	\caption{Decision tree of process $i$}
	\label{tree:VS}
\end{figure}

==> strategy.tex <==
% !TeX root = main.tex

In sections \ref{ssec:utility} and \ref{ssec:utilityCost}, we studied the existence of Nash equilibria in the game, considering particular strategies such that $\forall r \in  \mathbb{N}, \sigma^H(r) = \sigma^H(1)$.

When considering the case when we have $\exists r, r', r\neq r', \sigma^H(r) \neq \sigma^H(r')$, we have an infinite number of Nash equilibria, whatever the case we are studying.

\begin{theorem}\label{t:numberNEBlock}
	When considering the case when we have $\exists r, r', r\neq r', \sigma^H(r) \neq \sigma^H(r')$, whatever utility function is chosen, there are an infinite number of Nash equilibria.
\end{theorem}

\begin{proofT}
	
	\renewcommand{\toto}{t:numberNEBlock}
\end{proofT}

==> strategyVS.tex <==
% !TeX root = main.tex

In this section, we consider and analyse the situation where players have an action of checking the validity, and another action for sending the message.
The two action are not strictly independent. We note that if a player decides to check the validity of a message, and want to send the message, if the message is not valid, it does not send the message.

\begin{enumerate}
	\item If a player does not check the validity, it can send or not the message.
	\item If a player checks the validity of the message, it can send the message only if the message is valid.
\end{enumerate}
We note that if a message is valid, a player may decide to not send the message.

The algorithm that the players follow is depicted in Algorithm \ref{fig:protocol}.

The strategy of a player $\pi_i$ at a height $h$ is the following function $\sigma^h_i(r) = (\sigma^{h,\text{valid}}_i(r), \sigma^{h,\text{send}}_i(r))$ where:
$\sigma^{h,\text{valid}}_i: \mathbb{N}^* \to \{0,1\}$ and $\sigma^{h,\text{send}}_i: \mathbb{N}^* \to \{0,1\}$ are, respectively, the function that given a round let $\pi_i$ checks the validity and  sends a message.
When $h$ is clear from the context, we write $\sigma_i, \sigma^{\text{valid}}_i(r)$ and $\sigma^{\text{send}}_i(r))$.

In this section, we study the static case, and we assume that $\forall i \in \Pi, \forall r >0, \sigma_i(r) = \sigma_i(1)$.
Let $h > 0$ be a height:
\begin{itemize}
	\item $\sigma^h_i(r)$ is the strategy of the process $\pi_i$ during the height $h$, at the round $r$. Each strategy is composed of two actions, checking the validity of a message, and sending a message.
	\item $R$ is the round where the block has been produced \emph{i.e.} $\forall k: |\{ j : \sigma^{\text{send}}(k)=1\}| \ge \nu, R \le k$; it is the first round that satisfied the condition,
	\item $\Reward >0$ is the reward given once a block has been produced.
	\item an invalid block hurting the whole blockchain, we write $\invalidCost$ to represent that cost.
	\item $\costValid$ (resp. $\costSend$) represents the cost of checking the validity of (resp. sending) a message.
		We assume that $0 < \costSend , \costValid < \Reward < \invalidCost$.
	\item $\beta \in (0,1)$ is a discount factor, motivating the fact that if a block has been produced faster it worth more to the processes than if it is produced later.
	\item We note $p$ the probability of having an invalid block at a given height. We assume that it is a Bernoulli process such that in average the first round to have a valid block is $1/(1-p)$ \YAG{A voir si une autre distribution est meilleur}.
\end{itemize}

We assume here that messages are not lost. 
We study the memoryless strategies, such that $\pi_i$ has the same decision no matter the round of the previous behaviour of the other processes.


\begin{remark}
	If a player decides not to send a message, there is no point checking the validity\YAG{A prouver, mais pour chaque fonction d'utilite}
\end{remark}


Each player can choose one of the four following action :
\begin{itemize}
	\item Not Cheking the validity, and Not Send.
	\item Not Checking the validity and Send.
	\item Cheking the validity, and Not Send.
	\item Checking the validity and Send. We note that in this case, if the block is invalid, the player does not send the message.
\end{itemize}
	
	

	
